Machine Learning for Shipwreck Segmentation from Side Scan Sonar Imagery: Dataset and Benchmark

Open-source benchmark datasets have been a critical component for advancing machine learning for robot perception in terrestrial applications. Benchmark datasets enable the widespread development of state-of-the-art machine learning methods, which require large datasets for training, validation, and thorough comparison to competing approaches. Underwater environments impose several operational challenges that hinder efforts to collect large benchmark datasets for marine robot perception. Furthermore, a low abundance of targets of interest relative to the size of the search space leads to increased time and cost required to collect useful datasets for a specific task. As a result, there is limited availability of labeled benchmark datasets for underwater applications. We present the AI4Shipwrecks dataset, which consists of 28 distinct shipwrecks totaling 286 high-resolution labeled side scan sonar images to advance the state-of-the-art in autonomous sonar image understanding. We leverage the unique abundance of targets in Thunder Bay National Marine Sanctuary in Lake Huron, MI, to collect and compile a sonar imagery benchmark dataset through surveys with an autonomous underwater vehicle (AUV). We consulted with expert marine archaeologists for the labeling of robotically gathered data. We then leverage this dataset to perform benchmark experiments for comparison of state-of-the-art supervised segmentation methods, and we present insights on opportunities and open challenges for the field. The dataset and benchmarking tools will be released as an open-source benchmark dataset to spur innovation in machine learning for Great Lakes and ocean exploration. The dataset and accompanying software are available at https://umfieldrobotics.github.io/ai4shipwrecks/.

==> README <==
LaTeX package: forest [2017/07/14 v2.1.5 Drawing (linguistic) trees]

Copyright (c) 2012-2017 Saso Zivanovic
                   (Sa\v{s}o \v{Z}ivanovi\'{c})
saso.zivanovic@guest.arnes.si


ABSTRACT

`forest' is a pgf/tikz-based package for drawing linguistic (and other
kinds of) trees. Its main features are:
- a packing algorithm which can produce very compact trees;
- a user-friendly interface consisting of the familiar bracket
encoding of trees plus the key--value interface to option-setting;
- many tree-formatting options, with control over option values of
individual nodes and mechanisms for their manipulation;
- a powerful mechanism for traversing the tree;
- the possibility to decorate the tree using the full power of pgf/tikz;
- an externalization mechanism sensitive to code-changes.


LICENSE

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in

http://www.latex-project.org/lppl.txt

and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.


For the list of files constituting the work see the main source file
of the package, `forest.dtx', or the derived `forest.sty'.


